AI-Cybersecurity Education Through Designing AI-based Cyberharassment Detection Lab

Cyberharassment is a critical, socially relevant cybersecurity problem because of the adverse effects it can have on targeted groups or individuals. While progress has been made in understanding cyber-harassment, its detection, attacks on artificial intelligence (AI) based cyberharassment systems, and the social problems in cyberharassment detectors, little has been done in designing experiential learning educational materials that engage students in this emerging social cybersecurity in the era of AI. Experiential learning opportunities are usually provided through capstone projects and engineering design courses in STEM programs such as computer science. While capstone projects are an excellent example of experiential learning, given the interdisciplinary nature of this emerging social cybersecurity problem, it can be challenging to use them to engage non-computing students without prior knowledge of AI. Because of this, we were motivated to develop a hands-on lab platform that provided experiential learning experiences to non-computing students with little or no background knowledge in AI and discussed the lessons learned in developing this lab. In this lab used by social science students at North Carolina A&T State University across two semesters (spring and fall) in 2022, students are given a detailed lab manual and are to complete a set of well-detailed tasks. Through this process, students learn AI concepts and the application of AI for cyberharassment detection. Using pre- and post-surveys, we asked students to rate their knowledge or skills in AI and their understanding of the concepts learned. The results revealed that the students moderately understood the concepts of AI and cyberharassment.

==> Ethics.tex <==
\section{Ethical Statement}
We reflect on the ethical and privacy implications of our work due to its sensitive nature. When data was collected, no deleted, protected, or suspended accounts were included in our dataset as we adhered to Twitter's Standard API terms and Conditions (Twitter, Inc, 2022). Before our analyses (in 2023), we performed a non-compliance (e.g., deleted tweets or from suspended accounts) check of tweet IDs to ensure compliance with Twitter rules. All non-compliant tweets are excluded from our analyses. The example tweet quotations shown have been modified to protect the identity of the original author. Some content is offensive and sensitive; readers should read content cautiously.


==> PaperCheckList.tex <==
\section{AAAI ICWSM Paper Checklist}
\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    Yes
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    Yes
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    Yes
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    No
  \item Did you describe the limitations of your work?
    Yes
  \item Did you discuss any potential negative societal impacts of your work?
    NA
  \item Did you discuss any potential misuse of your work?
    NA
  \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
   NA
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
   Yes
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    NA
  \item Have you provided justifications for all theoretical results?
    NA
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    NA
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    NA
  \item Did you address potential biases or limitations in your theoretical framework?
    NA
  \item Have you related your theoretical results to the existing literature in social science?
    NA
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    NA
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    NA
	\item Did you include complete proofs of all theoretical results?
    NA
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    NA
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    NA
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    NA
   \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    NA
   \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    NA
   \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    NA
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    NA
  \item Did you mention the license of the assets?
    NA
  \item Did you include any new assets in the supplemental material or as a URL?
    NA
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    NA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    NA
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
NA
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
NA
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    NA
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    Yes
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    NA
   \item Did you discuss how data is stored, shared, and deidentified?
   NA
\end{enumerate}

\end{enumerate}
